CWCL: Cross-Modal Transfer with Continuously Weighted Contrastive Loss

This paper considers contrastive training for cross-modal 0-shot transfer wherein a pre-trained model in one modality is used for representation learning in another domain using pairwise data. The learnt models in the latter domain can then be used for a diverse set of tasks in a zero-shot way, similar to ``Contrastive Language-Image Pre-training (CLIP)'' and ``Locked-image Tuning (LiT)'' that have recently gained considerable attention. Most existing works for cross-modal representation alignment (including CLIP and LiT) use the standard contrastive training objective, which employs sets of positive and negative examples to align similar and repel dissimilar training data samples. However, similarity amongst training examples has a more continuous nature, thus calling for a more `non-binary' treatment. To address this, we propose a novel loss function called Continuously Weighted Contrastive Loss (CWCL) that employs a continuous measure of similarity. With CWCL, we seek to align the embedding space of one modality with another. Owing to the continuous nature of similarity in the proposed loss function, these models outperform existing methods for 0-shot transfer across multiple models, datasets and modalities. Particularly, we consider the modality pairs of image-text and speech-text and our models achieve 5-8% (absolute) improvement over previous state-of-the-art methods in 0-shot image classification and 20-30% (absolute) improvement in 0-shot speech-to-intent classification and keyword classification.

==> Content/author_response.tex <==
\newpage
\section{Author Response}

\textbf{Global response:}

We would like to thank all the reviewers for their time and effort in reviewing our paper. We appreciate all of the comments and they have helped us improve our paper. Here, we first provide a summary of our paper. Then, we outline the major concerns expressed by the reviewers and explain how we have addressed them. Following this, we also provide a summary of the positive comments made by the reviewers. 

\textbf{Paper summary:}
\begin{enumerate}
    \item We consider the problem of cross-modal transfer, where representations in one modality are learnt using a pre-trained model in another modality and a paired dataset that consists of pairs of the two modalities.
    \item To address inefficiencies in the training objective used in existing work, we propose a novel loss function called "Continuously Weighted Contrastive Loss" (CWCL) that considers associations between all the pairs in a training batch. 
    \item We show that the new loss function leads to 5-8\% (absolute) increase in 0-shot task performance for the image-text modality pair. We also study our method in the context of speech-text modality pair. We provide the first results in 0-shot speech-to-intent classification and keyword spotting, where our models achieve 20-30\% (absolute) improvement over existing methods.
\end{enumerate}

Overall, the reviewers has the following positive comments about our paper: The reviewers feel that our work addresses an important shortcoming in existing formulations ({\color{magenta}yjNF}, {\color{orange}1ozP})and that we propose a novel solution that is also simple and efficient ({\color{red}q9nH}). All the reviewers expressed that our experimental results are very strong. Reviewers also found the template-robustness property of our models interesting ({\color{teal}5jbW}).

\textbf{Summary of reviewer concerns}
We categorized the reviewers' concerns into broader themes. We describe them below provide a summary of our responses to each of them.

\textbf{Completeness of experiments and interpretation of the results:} Reviewer {\color{teal}5jbW } felt that some expreriments were missing for the image-text modality pair, {\color{magenta}yjNF} had some questions about experimental results, reviewer {\color{red}q9nH} had a question about the design choice for the similarity function, and {\color{orange}1ozP} asked for more results on the retrieval task for the image-text modality pair. We summarize our responses below:
\begin{itemize}
    \item We provide new experimental results in the rebuttal including a direct comparison between our method, CLIP and LiT on the retrieval task. We also provide updated results for all the image-text experiments with a new model architecutre based on the ViT-L-16+BERT-large configuration. 
    \item In particular, our new image-text model achieves a 0-shot ImageNet accuracy of 76.5\%, which is better than the best baseline (LiT) when trained on the same dataset.
    \item We have provided explanations for the choice of our baseline models in our response to reviewer {\color{magenta}yjNF}. We have also provided explanations for some of the results in Table 2 regarding the 0-shot performance in speech-text tasks.
    \item We have addressed why we chose the similarity function that we use in our paper. 
    \item We realized that we used two different naming conventions (`CL' and `LiT') for the baseline method that uses the standard contrastive learning loss. This lead to some confusion regarding the equivalence of the experiments between the image-text and speech-text modality pairs. We will correct this to ensure uniformity. 
\end{itemize}

\textbf{Comparison to existing work:} Reviewers {\color{magenta}yjNF} and {\color{red}q9nH} pointed us to a few papers that are relevant to our work. We provided details responses comparing our work to them in the rebuttal and we summarize it here.

All but one of the papers pointed out by the reviewers consider the weighted contrastive loss for \textbf{supervised learning}, where class information is available. In our work, we consider self-supervised learning. In the former case, conditioned on
prior information about which pairs are positive pairs and which are negative pairs, positive pairs that are further apart are weighted highly to bring them closer, and negative pairs that are closer are weighted highly so that they are pushed apart strongly. On the contrary, in our work, there is no notion of strictly positive or negative. This is a core contribution of the paper, since a softer notion of similarity helps us recreate the embedding space in one modality based on a pre-trained model from another modality. 

One of the papers considers self-supervised learning and is mroe similar to our paper. However, since they do not use pre-trained models, they need to use a "self-teaching" process, where a model is trained initially using only standard contrastive loss and then fine-tuned using a weighted contrastive loss.
During the rebuttal phase, we performed experiments with the self-teaching strategy and we found that that performance usually does not improve much or even degrades in our experiments. This maybe due to the conflicting nature of the two stages of training. We provide experimental results in our response. Further, The weighted loss they propose is designed to "down-weight" the effect of faulty positives and "up-weight" faulty negatives. In our method, we do not consider samples as positives or negatives.  

\textbf{Presentation of the paper:} We also received some comments about the presentation in our paper. We will address these concerns in the revised version of our paper. 


\textbf{Additional message to AC to ask if we can prompt the reviewer to respond:}

Dear AC(s),

We are writing to you to ask if we could post a new message to reviewer yjNF to provide some additional clarifications regarding their concerns. We were hoping to provide additional information once they respond to our rebuttal, but we have not heard from them. Hence, we wish to provide some more details that might result in a more engaging discussion with the reviewer and help us iterate over our clarifications further. The message we wish to write to them is below:

@@@ beginning of our message @@@

Dear reviewer, we wanted to provide some additional information to address some of your concerns. 

1. Comparison with "Not all negatives are equal..:" As previously mentioned, this paper considers the setting of supervised learning. In such a setting, the goal is to bring together the representations corresponding to data samples from the same class, while moving them away from other classes. Hence, there is a strict notion of \textbf{positive} and \textbf{negative} samples. Even though the paper studies a "weighting strategy", the goal of weights is to "apply stronger repulsive force to  more confusing negatives". Therefore, they only consider a summation over the "positive set" (as seen in Equation 3 of their paper). In this setting, an optimal solution is when all the data that belong to the same class are mapped to a single point, away from all other classes. 

On the contrary, in our setting, \textbf{we do not consider a strict notion of positive and negative}. The purpose of our weighting is to \textbf{reproduce the mutual relationships between data from one modality in another.} Hence, we consider a summation over all the data points in a training batch. 

We would like to emphasize that the difference between weighted contrastive loss and our setting might appear subtle, but the the two approaches differ significantly in their formulation and their outcomes. By design, the weighted loss function in the supervised setting \textbf{needs} "positive" and "negative" labels, whereas CWCL does not require any such supervision labels. It simply measures relationships between data samples using a continuos measure of similarity. As a result, the former can only perform classification on the classes in the supervised label set, whereas our models can perform zero-shot classification using relationships learnt using pre-trained models and similarity measures. 

However, we will cite this paper in our revised manuscript and provide a detailed comparison. 

2. Comparison with "Robust audio-visual instance discrimination": We already provided some details in our previous rebuttal. Additionally, we would also like to point out that we observe a large difference in performance of models trained with standard contrastive loss and CWCL in the case of speech-text modality pair. This further reinforces our hypothesis that the self-teaching strategy proposed in the above paper may not be the optimal way to go when strong pre-trained models are available. Pre-trained models not only result in better performance, but also lead to simpler weighting strategies as compared to those considered in the above paper. 


3. Please note that to the best of our knowledge, we are the first paper to study zero-shot methods for the speech-text modality pair. In this context, we show a strong difference in performance when we use CWCL. 

We are happy to provide any further information and are looking forward to discussing further with you.

@@@@ end of our message @@@@




\newpage 

\subsection{{\color{teal} Reviewer 1} (Score: 7)}

\begin{enumerate}

    \item{\color{blue} The ablation study comparing pure contrastive loss vs contrastive loss plus CWCL is only conducted for the audio-text alignment task. }

    Q: The ablation study...

    We provide the comparison between standard contrastive loss and CWCL for the image-text modality in Table. 1. Please note that we have chosen to name the standard contrastive loss based training as LiT, since we follow their training protocol by first initializing with a pre-trained image model and then using the standard contrastive loss as the training objective.
    
    The same comparison for the speech-text modality pair is provided in Table. 2. For standard contrastive loss, we initialize both speech and text encoders with pre-trained models, freeze them, and train the speech encoder only. In this regard, it is similar to LiT. However, we name this method as CL and not LiT, since LiT does not consider this pair of modalities, as its name suggests \textbf{L}ocked-\textbf{i}mage {\textbf{T}uning, and we wanted to avoid any misrepresentation of the LiT paper.
    
    Hence, the ablation studies presented in Table. 1 and 2. are equivalent and consider the image-text and speech-text modalities respectively. We will clarify this further in the revised paper.
    
    %We acknowledge that the difference in the names chosen to represent the standard contrastive loss and CWCL for the two cases might reduce readability. We will clarify this further in the revised paper. Please let us know if this clarified your concern. We are happy to present any further clarification if required. 



    % {\color{cyan} YMS: Do you think this question is because the reviewer missed that LiT = CL? Might be a good idea to clarify that here?}
        
    \item{\color{blue} In section 4.2.1, the author selected the text model very carefully. It thus seems that this method is very sensitive to the choice of the text model.} 

    Q: In section 4.2...
    
    We agree that the text model choice could affect the final model  performance in the downstream tasks. However, when selecting the two text models used in this paper, we simply selected 2 models that performed the best in the text intent classification on SLURP, among 50 publicly available text models (the details are written in 4.2's model architecture section). Please note the CWCL performance can be expected to be better than CL performance irrespective of the choice of the text model. We chose those text models to demonstrate good performance on downstream tasks. All that said, how to choose the right models for the training in detail is very much worth exploring in a separate work and we appreciate this comment.
    
    % In addition, the main focus of our paper is that CWCL outperforms vanilla CL in all those tasks although we tried our best to give explanations for the other results, too. The choice of text models affecting the performance is not limited to CWCL but is also applicable to CL.
    % {\color{green} JJ}
    % {\color{red}RS comments: We probably don't need to say it was simple and quick? We can maybe just emphasize that the difference between CWCL and CL can be expected for all models, but we also wanted to demonstrate the performance on good models and hence chose the models this way. }
    \item{\color{blue} It may provide more insight if there are some qualitative analyses between the model trained without CWCL and the model trained with CWCL.}

    Q: It may...
    
    In Figures 3, 7, and 8 in the original manuscript, we provide examples of the alignment between the audio and the text embeddings generated using the SLURP speech-to-intent classification dataset. Speech (audio) data in this dataset was never exposed to the model at any stage of training. In this figure, we can observe that using CWCL leads to a strong alignment between speech samples and text samples that have similar semantic meaning. For example, all the speech samples related to queries about the news have a high alignment with the text samples that have similar meaning. (We would like to emphasize that this alignment is observed in a downstream dataset whose speech data was not used during training.) However, we do not observe such an alignment in the models trained with only standard contrastive loss (CL), as seen in the figures. Hence, the speech embedding model trained with CWCL can be considered to have a better language understanding than one trained with CL. 

    A second set of qualitative results are provided in Section 4.1.2, where we study the robustness to templates in the image-text model. Owing to a stronger alignment between images and text, models trained using CWCL are able to generalize better under variations in the template sentences used. 
    
    % {\color{red} Provide some evidence in terms of paraphrased retrieval? This might also help with Reviewer 4's questions on retrieval.}

    % We appreciate the reviewer's question about qualitative analysis and we hope we have addressed this above. We are also open to any suggestions on other ways in which this can be demonstrated. 

    \item {\color{blue} The performance of LiT reported in Table 1 is much lower than the performance reported in the LiT paper. Could you explain what might be the reason for this discrepancy?} 

    Q: The perf...
    
    This is a good question! The mainis because of the architecture we used while training the models. In our experiments, we used the ViT-L/16 architecture for the image encoder and a 12 layer transformer for the text encoder. However, LiT achieves its best performance when the BERT-large architecture is used for the text encoder.
    
    In order to address this, we have now trained models using the ViT-L/16 + BERT-large configuration. We followed the training procedure described in the LiT paper as closely as possible. We provide results with the updated model architecture in Table \ref{tab:image-text-perf-bertlarge} (the PDF of the rebuttal). We are able to achieve much higher performance with the new architecture (LiT: 71.2\% , CWCL: 76.48\%). 

    Although we followd LiT's training protocol as closely as possible,the LiT model we trained achieves a zero-shot accuracy of 71.2\% on ImageNet (as opposed to 75.7\% mentioned in the LiT paper). We hypothesize that this difference is due to some training hyperparameters not fully specified in the LiT paper (such as the details of the Adafactor optimizer) and some possible differences in the training dataset (since some of the URLs in the CC12 and YFCC dataset may have become inactive, hence affecting our download of the dataset). However, under the same training setup, the CWCL model achieves 76.48\%.  In general, we again find that the CWCL-based models achieve much better performance. 

    % We hope we have addressed the reviewer's concern about the gap in LiT's reported performance and the performance we were able to achieve in our training. 

    \item {\color{blue} For the zero-shot keyword spotting task, because this task seems to be very much at the lexical level instead of the semantic level, I wonder what would be the benefit of using a contextualized pretrained language model? }

    Q: For the...
    
    We agree that the task of keyword spotting is at a lexical level than a semantic level. However, our goal is to train a versatile model that can be used for multiple tasks, e.g., speech-to-intent classification and keyword spotting.
    While using our model for keyword spotting, we convert the keywords to sentences and also convert the keyword classification task to the alignment task. This is similar to 0-shot image classification done by CLIP and LiT-like models, which is also a task that does not require contextual language information. Further, the contextualized pretrained language model could learn richer information in words considering the context in which each word is used. So our model performs well even when the keywords are used as is (without converting them to sentences).

    % {\color{cyan}JJ: I think some parts of what you said, we can add. However, in KWS, we not only converted the word into sentences based on the fixed templates (KWS\#) in some experiments but we also used the word (class label) as it is (KWS) in the other experiments, to get class embedding.}
    
    \item{\color{blue} Instead of having CWCL loss in addition to the original contrastive loss, what about having CWCL loss only but you set the weight of negative pairs to be 0? There seem to be some subtle design choices made for CWCL. I would like to know more.}

    Q: Instead...
    
    This is an interesting suggestion. When the weights for the negative pairs are set to 0, the resulting loss function is close to the standard loss function, except that the weights for the positive pairs can still be tuned. This might help with dealing with "faulty positives". We thank the reviewer for their suggestion. 

    In the current paper, we do not explore this and simply set the weights for the positive pairs to be 1, which results in the standard contrastive loss function. 


    
\end{enumerate}

\subsection{{\color{magenta} Reviewer 2} (Score: 5)}

\begin{enumerate}
    \item {\color{blue}The main contribution of this work (CWCL) can be grounded better in the context of existing work. This work highlights an important shortcoming in existing formulations of contrastive learning, namely that similarity has a binary interpretation. All positive examples and all negative examples are treated equally. This has been identified in prior work, albeit for a single modality, which the authors fail to cite. E.g., "Not All Negatives are Equal: Label-Aware Contrastive Loss for Fine-grained Text Classification", V. Suresh and D. Ong, EMNLP 2021. There are also works on multimodal learning that highlight the importance of using a weighted contrastive loss to downweight faulty positives/negatives such as "Robust Audio-Visual Instance Discrimination", Morgado et al., CVPR 2021.}

    Q: The main...
    
     Both references are very interesting and relevant and we will cite them.  We provide a detailed comparison below. 

     \textbf{Comparison with "Not all Negatives are Equal:.."}: 
     The ideas explored in this paper are similar in spirit to those considered in our paper. However, this paper considers supervised learning. In our work, we consider fully self-supervised learning. This lets us use our models on many downstream tasks in a zero-shot way, whereas in the supervised setting, the resulting models are applicable only to the specific task that they are trained for. 

     \textbf{Comparison with "Robust Audio-Visual Instance Discrimination" (soft-XID)}: 

    % This paper can be summarised as follows: The authors propose to align a video and an audio encoder by first training them with standard contrastive loss. After this first stage, they further train both the encoders using a weighted contrastive loss where they reduce the effect of faulty positives and negatives. Faulty positives are detected by measuring encoding corresponding video and audio frames using the encoders trained in the first stage. For any video-audio pair that has a poor alignment, the loss function term corresponding to that pair is weighted down. In doing so, such a data sample is \textit{effectively removed} from the training data (See equation 17 in the paper). For the pairs with a high alignment, the effect of faulty negatives is reduced by considering the alignment across all video and audio frames. 

     It is our belief that when models are trained initially using standard contrastive loss and then trained further by using weighted contrastive loss, biases from the initial training stage get further reinforced later on. In the initial stage of training, the encoders are are trained to repel all samples except only sample belonging to the same pair. When the same encoders are used to obtain the similarity scores in the second stage, these similarity scores are unreliable and will further reinforce the biases from the first stage.

     We performed an experiment that similar in spirit to the above paper. We trained a pair of image and text encoders using the standard constrative loss using the CC12M dataset for 20 epochs. Note that this is similar to the setup of the CLIP model. After this, we fine-tuned the model using weighted contrastive loss for another 20 epochs. In the second stage, we obtain the similarity scores using the encoders trained in the first stage, as proposed in "Robust ..." paper. We then measure the zero-shot image classification accuracy on ImageNet. We also train a model using the proposed CWCL method for a total of 40 epochs. We provide the results below in Table 11. We further note that in the first experiment (emulating soft-XID method) the 0-shot accuracy decreased upon fine-tuning, further indicating a conflict between the similarity scores generated using the models trained using standard constrastive loss. 

     Overall, we find that the method of first using standard constrastive loss and then using a weighted contrastive loss to yield worse performance as compared to our proposed method.
    

    \item {\color{blue} Did the authors experiment with other weighting functions for $w_ij$'s in Equation 3? Some insights on how $w_ij = q_i^T q_j/2 + 0.5$ was arrived at would be useful for the reader.}

    Q: Did...
    
We considered a softmax based weighting function defined as 
    \[ w_{i} \in \mathbb{R}^N := \text{softmax}(\langle q_i, q_k \rangle ),\ k = 1, \ \cdots \ N ,\]
     and $w_{i,j} = w_i[j]$ where the vector $w_i$ defines a distribution over the full training batch based on their inner products. 

     Secondly, we consider the function mentioned in our paper, where $w_{i,j}$ is given as 
     \[ w_{i,j} = \langle q_i , q_j\rangle/2 + 0.5 .\]

     The second formulation performs slightly better than the fist one. Further, it results in a nicer interpretation of the proposed CWCL loss function as an interpolation between standard contrastive loss and the supervised contrastive loss function, as mention in lines 130-134 in the main paper. 

     Further, note that in the second formulation, embeddings with $\langle q_i, q_j\rangle = -1$ result in a weight of 0, thus not resulting in any "attractive force" between such samples. 

    

    \item{\color{blue} As in Figure 5, does CWCL exhibit robustness to templates for the speech-to-intent classification task as well? } 

    Q: As in...
    
    Yes, we provide thein Table 10 of the rebuttal PDF. 
    
    
    \item {\color{blue}From Table 1, CWCL outperforms the supervised Resnet50 baseline on ImageNet-V2 as well as ImageNet-R, ImageNet-A and ObjNet by substantially larger margins. Is Resnet50 the appropriate supervised baseline to show for these datasets?}

    Q: From Table 1...

   One of the advantages of models such as CLIP, LiT and CWCL is that the same model can be used on multiple downstream tasks and datasets in a zero-shot way. To perform a more direct comparison to this regime, we choose a supervised and fine-tuned model that achieves a comparable performance on ImageNet and we report the same model's (after fine-tuning) accuracies on the other datasets. We wanted to better demonstrate how using a single model for multiple tasks performs and compare it with the CWCL-based model. Further, we also wish to note that the authors in \cite{zhai2022lit} make the same comparison.

    
    \item {\color{blue} From Table 2:
RoBERTa+S performs consistently better than BART+Y on SLURP and STOP, but the trend flips for KWS. Can the authors comment on why that is?} 

Q: From Table 2 RoBERTA+S...

The pre-trained text model used in RoBERTa+S was trained on the data including SLURP intent classification data (but only the text data. The SLURP speech data was not used in any stage of the training. Further, no data from STOP was used in the pre-training stage). We think that this affected the model to overfit on the task of intent classification in general, outperforming BART+Y (based on performances on SLURP and STOP) while performing worse in keyword spotting (KWS) than BART+Y.
% {\color{green} JJ}

% {\color{cyan} YMS: Replace last sentence as here? We think that this fine-tuning allowed the text model to learn better features geared towards intent classification than BART+Y (based on performances on SLURP and STOP). However, these features lead to worse performance in keyword spotting (KWS).}

% {\color{violet} RS: Can we also add this sentence after the first sentece: "Please note that only the text modality from SLURP was used in the pre-training of the RoBERTa+S language encoder. The speech data was not used in any stage of the training." (Reason being that it shouldn't make the reviewer suspicious about why we still call it zero-shot)}

% {\color{red} JJ: I've found that text-intent (upper bound) results in STOP (84.78 for RoBERTa+S, 92.93 BART+Y) are againt YMS's argument. If we only look at text-intent classification results, RoBERTa+S overfits to SLURP because it used the data as a part of its training data during FT. Thus, RoBERTa+S outperforms BART+Y in SLURP but underperforms it in STOP. However, in speech-intent classification RoBERTa+S always outperforms BART+Y. \\ I don't have any clear answer for this but roughly speaking, the embedding spaces for two text models are different and one could be more favorable when transferring the knowledge from text to speech. In our case, RoBERTa+S is more favorable than BART+Y. To support this, I checked the relative deduction in performance between text-intent and speech-intent when using CWCL. It was 27\% for RoBERTa+S and 31\% for BART+Y in SLURP. In STOP, I did not calculate it since the trend is more distinctively so (i.e., RoBERTa+S was more favorable than BART+Y again.). \\ That said, my final answer is as follows: CWCL with RoBERTa+S seems to tune the speech encoder more suitable to extract semantic information in a given speech at the cost of losing some of its ability to distinguish pronunciation that the pre-trained speech model originally had. (We think the pre-trained speech model has the ability to distinguish pronunciation since it was trained for ASR task that transcribes a given speech input where the ability to tell one pronunciation from the others is required.) In the case of the BART+Y-based system, it was simply trained worse (less) than the RoBERTa+S-based system for intent classification, so the extracted speech embedding retains more pronunciation information. This might have contributed to the result where CWCL w/ RoBERTa+S outpeformed the one w/ BART+Y in speech-intent classification (SLURP and STOP) while it was flipped in KWS.}


\item {\color{blue}From Table 2. CWCL with RoBERTa+S appears to outperform the text-intent upper bound for STOP (87.87 vs. 84.78). Please explain this result.}

Q: From Table 2 CWCL...

 We would like to clarify that in using the term "upper bound", we meant to convey that the text models' performance on intent classification serves as a "reference" for what can be expected from the speech encoder after training. We elaborate further below.

In our method, we "freeze" the text encoder and train the speech encoder using a paired (speech-text) dataset. In particular, we use the commonVoice datset. Note that the text model does not get updated and hence does not get a chance to process this dataset. Further, the speech encoder was initialized using a pre-trained ASR model's encoder. A third difference between the text model and the speech mode is that the speech tower might have learned how to utilize acoustic cues in addition to linguistic information from a given speech utterance, to align its embedding to the semantic embedding from the text tower.  These three differences could contribute to the speech model sometimes performing better than the text model. However, we still expect that the text model's performance to be a good reference for what the speech model can achieve after training. 

Another factor that might have lead to this is that the number of classes in the STOP dataset is low (8), as opposed to the SLURP dataset (which has 60 classes). Thus, in the case of SLURP, the performance on speech-intent task is lower than the text-intent task, since it is more challenging.

% We hope we have addressed the reviewer's concern. We will also update the paper with this clarification. 

% We've included the reason behind this result in the manuscript too, similar to what we answered here: During the cross-modal alignment stage using CWCL, the speech tower might have learned how to utilize acoustic cues in addition to linguistic information from a given speech utterance, to align its embedding to the semantic embedding from the text tower. Thus, the resulting speech tower utilizing the acoustic cues additionally could lead to better performance than the upper-bound text-intent classification performance in the specified result. However, this did not happen in SLURP since there are still some gaps between speech and text intent classification performances because SLURP data includes more intent classes than STOP (60 vs 8 classes), thus being more challenging in transferring knowledge from text to speech during the cross-modal alignment stage.
%Moreover, the STOP dataset only has 8 classes: 'weather', 'event', 'timer', 'alarm', 'music', 'messaging', 'navigation', and 'reminder' so this can be seen as an easier version of intent classification than SLURP. Thus, the performance gap between speech-to-intent and text-to-intent.
% (ratio uniq stn between stop vs slurp) 15228/2032, (ratio total stn) 33386/8691
 % {\color{green} JJ}

\end{enumerate}


\subsection{{\color{red}Reviewer 3 } (Score: 4)}

\begin{enumerate}
    \item {\color{blue} There is a lot of setup while the entirety of novel contributions seem to be buried in section 2.3. }

    Q: There is a...
    
    Please note the problem setup is only done in Section 2.1. We request the reviewer to elaborate further on what they mean by "lot of setup". 

    Further, our contributions are multi-fold and are not confined to Secton 2.3. The novel CWCL loss function is introduced in Section 2.2, while Section 2.3 discusses how we calculate the similarity weights. 

    Additionally, we demonstrate the effectiveness of the proposed methods using many experiments, models, datasets and modalitites. For example, we show the "template robustness" property of the proposed methods and we provide qualitative results showing that the proposed loss function leads to better alignment between the modalities. 

    We believe that this is the first work to study 0-shot speech-intent classification where no task-specific speech data was used for training. Further, our results show a strong improvement over methods that use standard contrastive loss. We would consider these results to be novel.

    In general, we request the reviewer to elaborate on why they feel that these other aspects are not novel. We believe that in a field like machine learning, an idea followed by extensive experimental results that demonstrate the effectiveness of the idea together contribute to novelty.

    \item {\color{blue} This paper makes more sense for a workshop, the contributions are limited and is a small modification of previous works such as \url{https://arxiv.org/pdf/1905.12837.pdf}, \url{https://arxiv.org/pdf/1811.01459.pdf}, \url{https://arxiv.org/pdf/2103.14003.pdf} }

Q: This paper...

\textbf{The General Pair-based Weighting Loss for Deep Metric Learning (\url{https://arxiv.org/pdf/1905.12837.pdf}):}

The referred paper is very different from ours for the following reasons:

Firstly, it studies the problem of metric learning in a supervised setting, where class information is available in the dataset. This is mentioned explicitly in Section 2.A of the paper where they formulate the problem and in Algorithm 1(authors mine “positive” and “negative” examples using Equations (16, 17) by using class labels). 


Secondly, they do not consider multi-modality. The algorithms proposed in this paper are geared towards a single modality. Hence, the resulting models cannot be used for other downstream tasks in a zero-shot way. On the contrary, they can only be used for the specific task that they are trained on. 

In our paper, we have already ackonwledged a weighted version of contrastive loss has been developed in the supervised learning case by Khosla et. al., (NeurIPS 2020, ref. [14] in our paper). However, extending weighted contrastive loss to self-supervised learning has not been studied before. Further, models such as CLIP and LiT have proven that scale of data and models have a large impact on downstream performance. But they only use the standard contrastive loss because developing a weighted contrastive loss in the context of they work was not explored before. Thus, our work is not a simple modification of the above paper.

\textbf{Deep Metric Learning by Online Soft Mining and Class-Aware Attention\url{https://arxiv.org/pdf/1811.01459.pdf}:}

This also addresses the problem of metric learning in a supervised setting. This is highlighted in the main methodology section, where they consider uni-modal dataset of the form ${x_i, y_i}$ where $y_i$ is the class label. This class label is used to define the positive set $P$ (samples with same class label) and negative set $N$ (samples with different class label), used compute the losses in eqns. (7, 8, 9).

\textbf{Rethinking Deep Contrastive Learning with Embedding Memory\url{https://arxiv.org/pdf/2103.14003.pdf}:}

This also addresses the supervised learning case; as we quotethe introduction section of above paper: “In this work, we simply adopt MoCo in a supervised manner for DML, which is referred as s-MoCo. It provides a strong example for us to study the pair weighting in memory-based DML”.


\textbf{Overall comments on comparison with the above three papers:}

We understand the reviewer’s concern that these papers study variations of weighted contrastive loss. However, extending weighted contrastive loss from a supervised setting to self-supervised setting is non-trivial. To summarize the difficulty, all the three papers pointed out consider the following question: Using prior information about positive and negative pairs, how to weight positive pairs that are further apart to bring them closer, and weight negative pairs that are closer so that they are pushed apart? This is captured in Figure 2. of the third paper pointed out by the reviewer (https://arxiv.org/pdf/2103.14003.pdf). Thus, an optimal solution here is where all positive samples are brought as close as possible, and all negative samples are pushed away as far as possible. On the contrary, in our work, there is no notion of strictly positive or negative. This is a core contribution of the paper, a softer notion of similarity helps us recreate the embedding space in one modality based on a pre-trained model from another modality. 
 
The difference between bringing together all positive samples and repelling all negative samples (with weighted or unweighted losses) and that of considering similarity as a continuous metric and learning a continuous structure in the embedding space of a modality  may be subtle, but the resulting algorithms and models have highly different capabilities and applications. Using supervised labels to construct positive and negative sets makes the models specific to those class labels; features that distinguish two inputs within a class are filtered out and features that distinguish two inputs from different classes are accentuated. However, since our models do not make use of class specific labels, they retain all features and are capable of zero-shot classification on many downstream tasks.

We hope we have addressed the reviewer’s concerns regarding the relationship between weighted contrastive loss in a supervised setting and our work and invite them for more discussion.  


    \item {\color{blue} Which continuous pairwise weights did the authors try? Given this is the main contribution it would be helpful to understand performance as this weighting changes in the 0.5 bias used or for nonlinear weighting wrt to the inner products. }

    Q: Which cont...
    
    Please refer to the answer we provided to Reviewer 2's questions on the different similarity functions that we considered and let us know if you have further questions. 
    
\end{enumerate}

\subsection{{\color{orange} Reviewer 4 } (Score: 5)}

\begin{enumerate}
    \item {\color{blue} The experimental results are not complete, it would be good to see a more complete set of results on how this method would perform on the downstream retrieval tasks (T4 compares between CL and CWCL, without indicating performance compared to baseline models such as LiT or CLIP). }

    Q: Results are incomplete...
    
    Thank you for raising this point. In Table 4, the row corresponding to `CL' is indeed the LiT model. We named it CL to indicate that this model was tuned using standard contrastive loss as done in the LiT paper. In fact, the model referred to in this row follows the same training procedure as LiT, with the image encoder initialized using a pre-trained model and frozen during training. We will make this change and rename the row to LiT to clarify this.

    Further, the results reported in the Table 4 correspond to using the ViT-L/16 architecture for the image encoder and a 12 layer transformer model for the text encoder; trained using the YFCC15M and the CC12M datasets. However, we noticed that LiT model achieves the best performance (using publicly available dataset) when BERT-large model is used as the text encoder.
    Thus, we performed further experiments with BERT-large model as the text encoder. We again observe an improvement in the retrieval performance. We provide the results in Table 12. Further, we also observe performance gains in the zero-shot image classification task as well. We provide the results in Table 13. 
    

    In the paper, we did not compare CWCL against CLIP on the retriaval task, since we expect CLIP to have lower performance than LiT (and CWCL already performs better than LiT). However, we realize that a direct comparison between CWCL and CLIP might be of interest. To this end, we provide a direct comparison of the two methods using zero-shot retrieval performance on MS-COCO dataset. Due to the limited time-frame, we trained new CWCL and CLIP models on a subset of the training data that consists of samples from/ only CC12M. Further, we trained both models for only 20 epochs. Although this setup is results in low absolute performance on both models, we can still obtain a direct relative comparison. We outline the results in Table 14. Interestingly, the models trained on CC12M dataset (Table 14) perform better at retrieval than models trained on both YFCC15M and CC12M (Table 4). We have noticed such behavior in open source CLIP models (\url{https://github.com/mlfoundations/open_clip}) as well. This we hypothesize is because CC12M is a dataset up that has been subject to filtering out bad samples, as opposed to YFCC15M which is not.


    % {\color{red} We will add the performance of the CLIP models trained using the same dataset and model architecture.}

    % Note that LiT paper reports an accuracy of 75.7\% zero-shot accuracy on Imagenet. However, we replicated their training as described in their paper and were able to obtain an accuracy of 71.2\%. In comparison, under the same setting, CWCl based model is able to achieve 76.48\%. Similarly, CWCL based model achieves much higher zero-shot accuracies on all the other datasets as well.

    

We hope that we have addressed the reviewer's concerns about results on retrieval task performance of CWCL based approach. We are happy to answer any further questions.


    \item {\color{blue} The experiments regarding the transfer from text to speech are nice however the results in Section 4.2.1 is not clearly presented and is a bit hard to follow.} 

    Q: Exp Text to Speech...
    
    Thank you for this comment. We reviewed and edited the entire section 4.2 carefully considering readers could be less familiar than us with the contents we wrote. We were also short on space and hence combined all results into a single table (Table 2 in the original manuscript). 
 In the revised paper, we will improve this section for readability. 
    
    % we changed some parts including Table 2 (modified version at Table~\ref{tab:ST-intent-kws-perf-rebuttal}) in the original manuscript to be more clearly presented. We can make this clear further given extra pages for camera-ready, e.g., by splitting the table.

    
    % {\color{green} JJ}

    \item {\color{blue} Figure1 is not really informative and maybe can be combined with Figure 4 so that more interesting and qualitative results can be presented.}

    Thank you for this suggestion. We will combine Figures 1 and 4. 
    % In particular, we will include the retrieval results and the results obtained using BERT-large encoder in the main manuscript. We welcome any suggestions on other results that can be included in the main paper.
    

    \item {\color{blue} Is it possible for you to provide results for retrieval compared to the baseline models? This would address a major weakness in the evaluation. }

    Q: Is it...

    We have provided the results on retrieval tasks in our response to one of your earlier comments. Further, we also provide results based on new experiments that studied the ViT-L-16+BERT-large configuration. We appreciate the reviewer's feedback regarding our experiments and we hope we have addressed their concern.

    
\end{enumerate}

Overall, we appreciate your questions and suggestions. They have helped us improve the paper. We agree that including performance on retrieval task adds to the completeness of our results. We will include these in the main paper manuscript. We will also clarify the results in Section 4.2.1. We were a little pressed for space in the original manuscript but we will better manage the space in the revised version by moving Figure 1. This will help us clarify the Section 4.2.1 further. 

We hope that we have addressed your concerns about our paper and sincerely hope to discuss further with you during the discussion phase. 


\newpage
\clearpage

\begin{table}
\parbox{.45\linewidth}{
    \centering
    \caption{Comparison for robustness to the number of sentence samples (k) used for class embedding generation. Reported numbers are relative accuracy reduction in zero-shot intent classification on SLURP (\%), relative to when all the training text samples are used for class embedding generation. k means the number of sentence samples from the \textit{train} subset of SLURP, used to generate each class embedding. The RoBERTa+S-based systems were compared.}
    \centering
    \label{tab:cmpr-nsample-robustness-rebuttal}
    \begin{tabular}{c|c|c|c}
    \toprule
         & k=1        & k=5        & k=10        \\
         \hline
    CL (baseline)  & 26.27 & 4.41   & 4.83  \\
    CWCL (ours) & 5.46 & 1.43 & 1.27  \\
    \bottomrule
    \end{tabular}
}
\hfill
\parbox{.45\linewidth}{
    \centering
    \caption{Comparison of the CWCL framework to the framework proposed in the paper by Morgado et. al. We train a pair of image and text encoders using the standard constrastive loss and then fine-tune it using a weighted version of the constrastive loss as described in their paper.}
    \label{tab:CL-then-CWCL}
    \begin{tabular}{c|c}
     \toprule
    Method & 0-shot ImageNet \\
    \midrule 
    soft-XID \cite{morgado2021robust} & 17.5\% \\
    \midrule 
    CWCL (Ours) & 69.83\%\\
      \bottomrule
    \end{tabular}
}
\end{table}

%     \begin{table}[h]
%     \caption{Comparison for robustness to the number of sentence samples used for class embedding generation. Reported numbers are relative accuracy reduction in zero-shot intent classification on SLURP (\%), relative to when all the training text samples are used for class embedding generation. k means the number of sentence samples from the \textit{train} subset of SLURP, used to generate each class embedding. The RoBERTa+S-based systems were compared.}
%     \centering
%     \label{tab:cmpr-nsample-robustness-rebuttal}
%     \begin{tabular}{c|c|c|c}
%     \toprule
%          & k=1        & k=5        & k=10        \\
%          \hline
%     CL (baseline)  & 26.27 & 4.41   & 4.83  \\
%     CWCL (ours) & 5.46 & 1.43 & 1.27  \\
%     \bottomrule
%     \end{tabular}
%     \end{table}


% \begin{table*}[th!]
%     \setlength{\tabcolsep}{5pt} % let TeX compute the
% \caption{In this table, we compare the CWCL framework to an approach similar to that proposed in the paper "Robust audio-visual instance discrimination". To do so, we first train a pair of image and text encoders using the standard constrastive loss and then fine-tune it using a weighted version of the constrastive loss as described in their paper.  }
% \label{tab:CL-then-CWCL}
% \begin{center}
% \begin{small}
% % \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{c|c}
%  \toprule
% Method & 0-shot ImageNet \\
% \midrule 
% soft-XID \cite{morgado2021robust} & 17.5\% \\
% \midrule 
% CWCL (Ours) & 69.83\%\\
%   \bottomrule
% \end{tabular}
% % }
% \end{small}
% \end{center}
% \end{table*}


    \begin{table*}[th!]
    \setlength{\tabcolsep}{5pt} % let TeX compute the
\caption{Zero-shot retrieval results on MS-COCO dataset by using ViT-L/16 and BERT-large model architectures as the image and text encoders respectively.}
\label{tab:MSCOCO_BERT}
\begin{center}
\begin{small}
% \resizebox{1\columnwidth}{!}{%
\begin{tabular}{c|ccc|ccc}
 \toprule
Method & \multicolumn{3}{c|}{I $\rightarrow$T retrieval} & \multicolumn{3}{c}{T$\rightarrow$I retrieval}\\
\midrule 
& R@1 & R@5 & R@10 & R@1 & R@5 & R@10 \\
\midrule 
LiT & 34.58 & 59.78 & 70.68 & 28.49 & 54.04 & 65.87 \\
\midrule 
\textbf{CWCL (Ours)} & \textbf{40.36} & \textbf{66.62} & \textbf{77.76} & \textbf{30.04} & \textbf{54.84} & \textbf{66.06}\\
  \bottomrule
\end{tabular}
% }
\end{small}
\end{center}
\end{table*}

\begin{table*}[th!]
\setlength{\tabcolsep}{5pt} % let TeX compute the
\caption{Zero-shot image classification using a model with\textbf{ ViT-L/16} based image encoder and a \textbf{BERT-large} based text encoder trained on a combination of CC12M and YFCC datasets. \textit{CWCL-based training achieves state-of-the-art performance on all of zero-shot experiments.}}
\vspace{-0.3cm}
\label{tab:image-text-perf-bertlarge}
\begin{center}
\begin{small}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{cccccc}
 \toprule
  Method & ImageNet (\%) & ImageNet-V2(\%) & ImageNet-R(\%) & ImageNet-A(\%) & ObjNet(\%) \\ 
 \midrule 
  LiT & 71.2 & 62.98 & 63.8 & 40.28 & 48.1 \\
 \textbf{CWCL (Ours)} & \textbf{76.48} & \textbf{67.86} & \textbf{68.7} & \textbf{47.27}& \textbf{52.38}\\
 \bottomrule
\end{tabular}
}
\end{small}
\end{center}

\end{table*}


    \begin{table*}[th!]
    \setlength{\tabcolsep}{5pt} % let TeX compute the
\caption{Small experiment (models trained on CC12M dataset for 20 epochs) to compare CWCL and CLIP for zero-shot retrieval on MS-COCO dataset (Image: ViT-L/16, Text: 12-layer transformer).}
\label{tab:CWCL-CLIP-MSCOCO}
\begin{center}
\begin{small}
% \resizebox{1\columnwidth}{!}{%
\begin{tabular}{c|ccc|ccc}
 \toprule
Method & \multicolumn{3}{c|}{I $\rightarrow$T retrieval} & \multicolumn{3}{c}{T$\rightarrow$I retrieval}\\
\midrule 
& R@1 & R@5 & R@10 & R@1 & R@5 & R@10 \\
\midrule 
CLIP & 14.2 & 32.1 & 44.32 & 8.83 & 23.63 & 33.36\\
\midrule 
\textbf{CWCL (Ours)} & \textbf{38.48} & \textbf{65.62} & \textbf{76.6} & \textbf{26.79} & \textbf{51.76} & \textbf{63.37}\\
  \bottomrule
\end{tabular}
% }
\end{small}
\end{center}
\end{table*}    
    


% \begin{table}[t]
% \renewcommand{\arraystretch}{1}
%   \caption{Top-1 accuracy for zero-shot speech-to-intent classification (SLURP and STOP) and keyword spotting (GSCV2) after thick vertical line. Superscript $^\#$ is used to indicate use of general templates for class embedding extraction. Supervised results are provided in \textcolor{gray}{gray} after the double-horizontal line: \cite{arora2022espnet} is for speech-to-intent and \cite{de2018neural, baevski2020wav2vec, niizumi2023masked} are for keyword spotting.}
%   \label{tab:ST-intent-kws-perf-rebuttal}
%   \centering
%   \begin{small}
%   \begin{tabular}{cc|cc|cc?cc}
%  \hline
%  Method & Text model & SLURP & SLURP$^\#$ & STOP & STOP$^\#$  & GSCV2 & GSCV2$^\#$ \\
%  \midrule
% CL &  RoBERTa+S & 40.35 & 23.68 & 70.13 & 50.56 & 64.74 & 59.65 \\
% (baseline) &  BART+Y & 22.73 & 8.06 & 55.67 & 42.07 & 56.33 & 45.54\\ 
% \hline
% \textbf{CWCL} & RoBERTa+S & 63.80 & 40.75 & 87.87 & 67.77 & 81.02 & 82.77 \\
% \textbf{(Ours)} & BART+Y & 53.12 & 30.51 & 80.99 & 73.08 & 88.81 & 89.43\\
%  \hline
% Text-intent & RoBERTa+S & 88.19 & 59.86 & 84.78 & 69.10 & 100 & 98.20 \\
% (upper bound) & BART+Y & 77.03 & 45.93 & 92.93 & 79.11 & 100 & 100\\
%  \hline
%  \hline
%  \textcolor{gray}{ESPnet} \cite{arora2022espnet} & - & \textcolor{gray}{77.00} & - & - & - & - & - \\
% %\hline
% \textcolor{gray}{Att. RNN} \cite{de2018neural} & - & - & - & - & - & \textcolor{gray}{93.9} & - \\
%  % \textcolor{gray}{KWT-2} \cite{berg2021keyword} & - & \textcolor{gray}{(97.74, -)} & -  \\
%  \textcolor{gray}{Wav2Vec2} \cite{baevski2020wav2vec} & - & - & - & - & - & \textcolor{gray}{96.6} & -  \\
%  % \textcolor{gray}{M2D} \cite{niizumi2023masked} & - & \textcolor{gray}{(95.4, -)} & -  \\
%  \textcolor{gray}{M2D} \cite{niizumi2023masked} & - & - & - & - & - & \textcolor{gray}{98.5} & -  \\
%  \bottomrule
% \end{tabular}
% \end{small}
% \vspace{-4mm}
% \end{table}



==> Content/refrence_list.tex <==
[1] [DONE] L. Wu, C. Wu, H. Guo, and Z. Zhao, “A Cross-Modal Alignment for Zero-Shot Image Classification,” IEEE Access, vol. 11, pp. 9067–9073, 2023, doi: 10.1109/ACCESS.2023.3237966.
[2] [DONE] J. Wehrmann, C. Kolling, and R. C. Barros, “Adaptive Cross-Modal Embeddings for Image-Text Alignment,” Proceedings of the AAAI Conference on Artificial Intelligence, vol. 34, no. 07, Art. no. 07, Apr. 2020, doi: 10.1609/aaai.v34i07.6915.
[3] [DONE] J. Li, R. R. Selvaraju, A. D. Gotmare, S. Joty, C. Xiong, and S. Hoi, “Align before Fuse: Vision and Language Representation Learning with Momentum Distillation.” arXiv, Oct. 07, 2021. doi: 10.48550/arXiv.2107.07651.
[4] [DONE] Z. Novack, S. Garg, J. McAuley, and Z. C. Lipton, “CHiLS: Zero-Shot Image Classification with Hierarchical Label Sets.” arXiv, Feb. 06, 2023. doi: 10.48550/arXiv.2302.02551. %This has good references in the beginning for CLIP like papers.
[5] [DONE] B. Elizalde, S. Deshmukh, M. A. Ismail, and H. Wang, “CLAP Learning Audio Concepts from Natural Language Supervision,” in ICASSP 2023 - 2023 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP), Jun. 2023, pp. 1–5. doi: 10.1109/ICASSP49357.2023.10095889.
[6] [DONE] J. Yu, Z. Wang, V. Vasudevan, L. Yeung, M. Seyedhosseini, and Y. Wu, “CoCa: Contrastive Captioners are Image-Text Foundation Models.” arXiv, Jun. 13, 2022. doi: 10.48550/arXiv.2205.01917.
[7] [DONE] I. Manco, E. Benetos, E. Quinton, and G. Fazekas, “Contrastive Audio-Language Learning for Music.” arXiv, Aug. 25, 2022. doi: 10.48550/arXiv.2208.12208.
[8] [DONE] R. Ye, M. Wang, and L. Li, “Cross-modal Contrastive Learning for Speech Translation.” arXiv, May 05, 2022. doi: 10.48550/arXiv.2205.02444.
[9] [DONE] M. Zolfaghari, Y. Zhu, P. Gehler, and T. Brox, “CrossCLR: Cross-modal Contrastive Learning For Multi-modal Video Representations,” in 2021 IEEE/CVF International Conference on Computer Vision (ICCV), Montreal, QC, Canada: IEEE, Oct. 2021, pp. 1430–1439. doi: 10.1109/ICCV48922.2021.00148.
[10] [DONE] J.-B. Alayrac et al., “Flamingo: a Visual Language Model for Few-Shot Learning,” Advances in Neural Information Processing Systems, vol. 35, pp. 23716–23736, Dec. 2022.
[11] [NOT RELEVANT] A. Steiner, A. Kolesnikov, X. Zhai, R. Wightman, J. Uszkoreit, and L. Beyer, “How to train your ViT? Data, Augmentation, and Regularization in Vision Transformers.” arXiv, Jun. 23, 2022. doi: 10.48550/arXiv.2106.10270.
[12] [NOT RELEVANT] C. Schuhmann et al., “LAION-5B: An open large-scale dataset for training next generation image-text models.” arXiv, Oct. 15, 2022. doi: 10.48550/arXiv.2210.08402.
[13] [THIS IS THE CLIP PAPER] A. Radford et al., “Learning Transferable Visual Models From Natural Language Supervision.” arXiv, Feb. 26, 2021. doi: 10.48550/arXiv.2103.00020.
[14] [DONE] B. Mustafa, C. Riquelme, J. Puigcerver, R. Jenatton, and N. Houlsby, “Multimodal Contrastive Learning with LIMoE: the Language-Image Mixture of Experts.” arXiv, Jun. 06, 2022. doi: 10.48550/arXiv.2206.02770.
[15] [DONE] Z. Lin, S. Yu, Z. Kuang, D. Pathak, and D. Ramanan, “Multimodality Helps Unimodality: Cross-Modal Few-Shot Learning with Multimodal Models.” arXiv, Jan. 29, 2023. doi: 10.48550/arXiv.2301.06267.
[16] [NOT NEEDED] M. Cherti et al., “Reproducible scaling laws for contrastive language-image learning.” arXiv, Dec. 14, 2022. doi: 10.48550/arXiv.2212.07143.
[17] [DONE] X. Zhai, B. Mustafa, A. Kolesnikov, and L. Beyer, “Sigmoid Loss for Language Image Pre-Training.” arXiv, May 04, 2023. doi: 10.48550/arXiv.2303.15343.
[18] [DONE] Y. Patel, Y. Xie, Y. Zhu, S. Appalaraju, and R. Manmatha, “SimCon Loss with Multiple Views for Text Supervised Semantic Segmentation.” arXiv, Feb. 07, 2023. doi: 10.48550/arXiv.2302.03432.
[19] [DONE] M. Shu et al., “Test-Time Prompt Tuning for Zero-Shot Generalization in Vision-Language Models.” arXiv, Sep. 15, 2022. doi: 10.48550/arXiv.2209.07511.
[20] [DONE] C. Wu, S. Yin, W. Qi, X. Wang, Z. Tang, and N. Duan, “Visual ChatGPT: Talking, Drawing and Editing with Visual Foundation Models.” arXiv, Mar. 08, 2023. doi: 10.48550/arXiv.2303.04671.

%% New Refs added
[21] [DONE] Yang, Jianwei, Chunyuan Li, Pengchuan Zhang, Bin Xiao, Ce Liu, Lu Yuan, and Jianfeng Gao. "Unified contrastive learning in image-text-label space." In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition, pp. 19163-19173. 2022.
% A novel extension to Contrastive loss. 
[22] [DONE] Guzhov A, Raue F, Hees J, Dengel A. Audioclip: Extending clip to image, text and audio. InICASSP 2022-2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP) 2022 May 23 (pp. 976-980). IEEE.
[23] [DONE] Wu HH, Seetharaman P, Kumar K, Bello JP. Wav2clip: Learning robust audio representations from clip. InICASSP 2022-2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP) 2022 May 23 (pp. 4563-4567). IEEE.
% CLAP says for [22] and [23] they cannot do zero-shot.
[24] [DONE] Arora, Sanjeev, Hrishikesh Khandeparkar, Mikhail Khodak, Orestis Plevrakis, and Nikunj Saunshi. "A theoretical analysis of contrastive unsupervised representation learning." arXiv preprint arXiv:1902.09229 (2019).
[25] [DONE] Sohn, K., Li, C.L., Yoon, J., Jin, M. and Pfister, T., Learning and Evaluating Representations for Deep One-Class Classification. In International Conference on Learning Representations.
[26] [DONE] Chuang, C.Y., Robinson, J., Lin, Y.C., Torralba, A. and Jegelka, S., 2020. Debiased contrastive learning. Advances in neural information processing systems, 33, pp.8765-8775.
